Commit0: Library Generation from Scratch

With the goal of benchmarking generative systems beyond expert software development ability, we introduce Commit0, a benchmark that challenges AI agents to write libraries from scratch. Agents are provided with a specification document outlining the library's API as well as a suite of interactive unit tests, with the goal of producing an implementation of this API accordingly. The implementation is validated through running these unit tests. As a benchmark, Commit0 is designed to move beyond static one-shot code generation towards agents that must process long-form natural language specifications, adapt to multi-stage feedback, and generate code with complex dependencies. Commit0 also offers an interactive environment where models receive static analysis and execution feedback on the code they generate. Our experiments demonstrate that while current agents can pass some unit tests, none can yet fully reproduce full libraries. Results also show that interactive feedback is quite useful for models to generate code that passes more unit tests, validating the benchmarks that facilitate its use.

==> qualitative.tex <==
% We collect X(change later) common cases where agent successful make correct changes.

% Type 1: Correctly implement the function explicitly with "pass" in implementation. For example in cachetools --->. We 


% % src/cachetools/keys.py
% % ```python
% % <<<<<<< SEARCH
% % def hashkey(*args, **kwargs):
% %     """Return a cache key for the specified hashable arguments."""
% %     pass
% % =======
% % def hashkey(*args, **kwargs):
% %     """Return a cache key for the specified hashable arguments."""
% %     if kwargs:
% %         return _HashedTuple(args + sum(sorted(kwargs.items()), _kwmark))
% %     else:
% %         return _HashedTuple(args)
% % >>>>>>> REPLACE
% % ```

% % src/cachetools/keys.py
% % ```python
% % <<<<<<< SEARCH
% % def methodkey(self, *args, **kwargs):
% %     """Return a cache key for use with cached methods."""
% %     pass
% % =======
% % def methodkey(self, *args, **kwargs):
% %     """Return a cache key for use with cached methods."""
% %     return hashkey(self.__class__, *args, **kwargs)
% % >>>>>>> REPLACE
% % ```

% % src/cachetools/keys.py
% % ```python
% % <<<<<<< SEARCH
% % def typedkey(*args, **kwargs):
% %     """Return a typed cache key for the specified hashable arguments."""
% %     pass
% % =======
% % def typedkey(*args, **kwargs):
% %     """Return a typed cache key for the specified hashable arguments."""
% %     key = hashkey(*args, **kwargs)
% %     return _HashedTuple(tuple(type(arg) for arg in args) + (key,))
% % >>>>>>> REPLACE
% % ```

% % src/cachetools/keys.py
% % ```python
% % <<<<<<< SEARCH
% % def typedmethodkey(self, *args, **kwargs):
% %     """Return a typed cache key for use with cached methods."""
% %     pass
% % =======
% % def typedmethodkey(self, *args, **kwargs):
% %     """Return a typed cache key for use with cached methods."""
% %     key = methodkey(self, *args, **kwargs)
% %     return _HashedTuple((self.__class__,) + tuple(type(arg) for arg in args) + (key,))
% % >>>>>>> REPLACE
% % ```


% this will give 
% % ============================= test session starts ==============================
% % platform linux -- Python 3.10.12, pytest-8.3.3, pluggy-1.5.0
% % rootdir: /testbed
% % configfile: pyproject.toml
% % plugins: json-report-1.5.0, metadata-3.1.1, cov-5.0.0
% % collected 5 items

% % tests/test_keys.py .....                                                 [100%]

% % --------------------------------- JSON report ----------------------------------
% % report saved to: report.json
% % ============================== 5 passed in 0.03s ===============================

% % >  
% % > cls = <class 'tests.test_sphinx_metaclass.ClassicAdapter._decorate_class.<locals>.NewClass'>  
% % > a = 'five', b = 5  
% % >  
% % > def __new__(cls, a, b=5):  
% % > >       obj = super(MyClass, cls).__new__(cls)  
% % > E       TypeError: test_with_new.<locals>.MyClass.__new__() missing 1 required positional argument: 'a'  
% % >  
% % > tests/test_sphinx_metaclass.py:45: TypeError  
% % > --------------------------------- JSON report ----------------------------------  
% % > report saved to: report.json  
% % > =========================== short test summary info ============================  
% % > FAILED tests/test_sphinx_metaclass.py::test_with_new - TypeError: test_with_n...  
% % > ========================= 1 failed, 3 passed in 0.14s ==========================  
% % >  


% Type 2: Test provides important information.

% We collect X(change later) common errors agent produced. 

% Type 1: Model failed to commit the change

% Type 2: Lint introduce error: Sometimes lint error will give error like "#### deprecated/classic.py:74:24: ANN001 Missing type annotation for function argument `reason`" and then the agent will update the type for the varibale. However, the type it added to the variable might not be successfully import, such as Callable and Any. 

% % deprecated/classic.py
% % ```python
% % <<<<<<< SEARCH
% %     def __call__(self, wrapped):
% % =======
% %     def __call__(self, wrapped: Callable) -> Callable:
% % >>>>>>> REPLACE
% % ```

% % -> NameError: name 'Callable' is not defined.

% This error might be further caught by lint error itself, but there are only 3 max reflections by default, so in some cases the agent just make the changes and proceed to next file.

% Type 3: Agent changed test file, which is not allowed.

% Type 4: Model failed to write imported method in another file

% Type 4: 
